Text Descriptions are Compressive and Invariant Representations for Visual Learning

Modern image classification is based upon directly predicting classes via large discriminative networks, which do not directly contain information about the intuitive visual features that may constitute a classification decision. Recently, work in vision-language models (VLM) such as CLIP has provided ways to specify natural language descriptions of image classes, but typically focuses on providing single descriptions for each class. In this work, we demonstrate that an alternative approach, in line with humans' understanding of multiple visual features per class, can also provide compelling performance in the robust few-shot learning setting. In particular, we introduce a novel method, \textit{SLR-AVD (Sparse Logistic Regression using Augmented Visual Descriptors)}. This method first automatically generates multiple visual descriptions of each class via a large language model (LLM), then uses a VLM to translate these descriptions to a set of visual feature embeddings of each image, and finally uses sparse logistic regression to select a relevant subset of these features to classify each image. Core to our approach is the fact that, information-theoretically, these descriptive features are more invariant to domain shift than traditional image embeddings, even though the VLM training process is not explicitly designed for invariant representation learning. These invariant descriptive features also compose a better input compression scheme. When combined with finetuning, we show that SLR-AVD is able to outperform existing state-of-the-art finetuning approaches on both in-distribution and out-of-distribution performance.

==> experiment_old.tex <==
\section{Experiment}

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_ind.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_r.pdf}

     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_a.pdf}

     \end{subfigure}
     
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_v2.pdf}

     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_sketch.pdf}

     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_object.pdf}

     \end{subfigure}
        \caption{Few-shot experiments compare LP vs SLR-AVD. In each subfigure, the y-axis represents the number of shots per class. Here we consider shot in $[1,2,4,8,16,32]$ per class. SLR-AVD is more sample efficient in the in-distribution reference and is also much more robust to several distribution shifts.}
        \label{fig:fs_comparison}
\end{figure*}


Throughout the experiments, we focus on the few-shot setting. We test our method on ImageNet,  ImageNet-R, ImageNet-V2, ImageNet-A, ImageNet-Sketch, and ObjectNet \citep{deng2009imagenet,hendrycks2021many,hendrycks2021natural,recht2019imagenet,wang2019learning,barbu2019objectnet}, demonstrating the superiority of the learned ensemble over visual descriptors. By default, we use the ViT-B/16 model unless otherwise specified. The hand-crafted templates for ImageNet classes contain a set of seven prompts suggested in \href{https://github.com/openai/CLIP}{https://github.com/openai/CLIP}:
\begin{enumerate*}[series = tobecont, itemjoin =\quad]
	\item ``\texttt{itap of a \{\}.}''
	\item ``\texttt{a bad photo of the  \{\}.}''
	\item ``\texttt{a origami \{\}.}''
	\item ``\texttt{a photo of the large \{\}.}'
	\item ``\texttt{a \{\} in a video game.}''
    \item ``\texttt{art of the \{\}.}''
	\item ``\texttt{a photo of the small \{\}.}''
\end{enumerate*} 
This set usually outperforms the original $80$ templates in \citet{radford2021learning}.




%\begin{table*}[h!]
%\centering
% \begin{tabular}{lc|ccccc} 
% \midrule
% & IN (reference) & IN-V2 & IN-R & IN-A & IN-Sketch & ObjectNet \\ [0.5ex] 
%\midrule
%\texttt{CLIP ViT-L/14@336px} & & & & & & \\
%\quad Zero-shot \citep{menon2022visual} & 72.97 & 66.58 & -- & -- & -- & -- \\ 
%\quad  Visual descriptor (VD) \citep{menon2022visual} & 76.16 & 70.32 & -- & -- & -- & --  \\
%\quad Zero-shot \citep{wortsman2022robust} & 76.7 & 70.5 & 89.0 & 77.7 & 60.9 & 69.1\\
%\quad  Zero-shot (Our) & 76.61 & 70.78 & 89.05 & 77.65 & 60.76 & 68.75\\
%\quad  VD (our) & 73.58 & 68.35 & 85.57 & 72.72 & 56.78 & 63.58\\
%\quad  Augmented VD & \textbf{77.24} & \bf 71.67 & \bf 89.27 & \bf 78.27 & \bf 61.25 & \bf 69.14\\ [1ex] 
%
%\midrule
%\texttt{CLIP ViT-B/16} & & & & & & \\
%\quad  Zero-shot (Our) & 68.78 & 62.23 & 77.72 & 50.64 & 48.38 & 54.31\\
%\quad  VD (our) & 65.89 & 59.19 & 72.75 & 46.11 & 44.84 & 49.60\\
%\quad  Augmented VD & \textbf{69.52} & \bf 62.97 & \bf 77.85 & \bf 50.87 & \bf 48.91 & \bf 54.58\\ [1ex] 
%
% \bottomrule
% \end{tabular}
% \caption{Accuracies of zero-shot, visual descriptors, and augmented visual descriptors on ImageNet and its variation. Experiments are done on ViT-L/14@336px and ViT-B/16 models, and AVD outperforms all baselines across different datasets and models.}
% \label{table:zs_comparison}
%\end{table*}


%\begin{table}[h!]
%\centering
% \begin{tabular}{c|ccc} 
% \midrule
% & ZS & ZS-VD & ZS-AVD \\
% \midrule
% IN & 68.78 & 65.89 & \bf 69.52\\ 
% IN-V2 & 62.23 & 59.19 & \bf 62.97\\ 
% IN-R & 77.72 & 72.75 & \bf 77.85\\ 
% IN-A & 50.64 & 46.11 &\bf  50.87\\ 
% IN-Sketch & 48.38 & 44.84 & \bf 48.91\\ 
% ObjectNet & 54.31 & 49.60 &\bf  54.58\\ 
% \bottomrule
% \end{tabular}
% \caption{Accuracies of zero-shot, visual descriptors, and augmented visual descriptors on ImageNet and its variation. ZS-AVD outperforms all baselines across different datasets.}
% \label{table:zs_comparison}
%\end{table}
%
%\begin{table}[h!]
%\centering
%%\resizebox{\columnwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c} 
% \toprule
% Shot&  \multicolumn{2}{c|}{$k=1$} & \multicolumn{2}{c|}{$k=2$} & \multicolumn{2}{c}{$k=4$}\\
% \midrule
%Method& FT & SLR & FT & SLR &FT & SLR\\
%\midrule
%IN & 68.88 & 70.31 & 69.59 & 71.21 & 70.48 & 72.09\\
%\midrule
%Average $\uparrow$ &  \multicolumn{2}{c|}{1.43} &  \multicolumn{2}{c|}{1.62} &  \multicolumn{2}{c}{1.61}\\
%\midrule
%IN-R & 77.82 & 78.29 & 78.13 & 78.53 & 78.32 & 78.59\\
%IN-A & 50.09 & 51.29 & 50.43 & 51.51 & 52.11 & 52.64 \\
%IN-V2 & 62.32 & 63.74 & 63.07 & 64.37 & 63.50 & 65.30\\
%IN-Sketch & 48.45 & 49.35 & 48.75 & 49.63 & 48.99 & 49.92\\
%ObjectNet & 54.52 & 54.94 & 55.01 & 54.99 & 55.77 & 55.41\\
%\midrule
%Average $\uparrow$ &  \multicolumn{2}{c|}{0.88} &  \multicolumn{2}{c|}{0.73} &  \multicolumn{2}{c}{0.64}\\
%\bottomrule
% \end{tabular}
%% }
% \caption{Accuracies on ImageNet and its variation with the optimal choice of $\alpha$. We compare WISE-FT to WISE-SLR.}
% \label{table:optimal_alpha_ft}
%\end{table}



\begin{figure}[htb]
\centering
\begin{minipage}[t]{0.55\textwidth}\vspace{0pt}\centering
 \captionof{table}{Accuracies on ImageNet and its variation with the optimal choice of $\alpha$. We compare WISE-FT to WISE-SLR.}
\resizebox{\columnwidth}{!}{
 \begin{tabular}{c|c|c|c|c|c|c} 
 \toprule
 Shot&  \multicolumn{2}{c|}{$k=1$} & \multicolumn{2}{c|}{$k=2$} & \multicolumn{2}{c}{$k=4$}\\
 \midrule
Method& FT & SLR & FT & SLR &FT & SLR\\
\midrule
IN & 68.88 & 70.31 & 69.59 & 71.21 & 70.48 & 72.09\\
\midrule
Average $\uparrow$ &  \multicolumn{2}{c|}{1.43} &  \multicolumn{2}{c|}{1.62} &  \multicolumn{2}{c}{1.61}\\
\midrule
IN-R & 77.82 & 78.29 & 78.13 & 78.53 & 78.32 & 78.59\\
IN-A & 50.09 & 51.29 & 50.43 & 51.51 & 52.11 & 52.64 \\
IN-V2 & 62.32 & 63.74 & 63.07 & 64.37 & 63.50 & 65.30\\
IN-Sketch & 48.45 & 49.35 & 48.75 & 49.63 & 48.99 & 49.92\\
ObjectNet & 54.52 & 54.94 & 55.01 & 54.99 & 55.77 & 55.41\\
\midrule
Average $\uparrow$ &  \multicolumn{2}{c|}{0.88} &  \multicolumn{2}{c|}{0.73} &  \multicolumn{2}{c}{0.64}\\
\bottomrule
 \end{tabular}
}

 
 \label{table:optimal_alpha_ft}
\end{minipage}

\end{figure}


\begin{figure*}[htbp]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wiseft_avg_shot4}

     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wiseft_avg_shot8}

     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wiseft_avg_shot16}

     \end{subfigure}

        \caption{ID-OOD accuracy curve of weight ensemble of LP vs weight ensemble of SLR-AVD. ID is tested on ImageNet, and OOD is averaged over $5$ ImageNet variations. Experiments with $[4,8,16]$-shots are presented. Each accuracy is averaged over $3$ runs. We can see that our proposed method overwhelms LP in all cases.}
        \label{fig:id_ood_curve_avg}
\end{figure*}

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wiseft_avg_ft_shot1}

     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wiseft_avg_ft_shot2}

     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wiseft_avg_ft_shot4}

     \end{subfigure}

        \caption{ID-OOD accuracy curve of WISE-FT vs WISE-SLR. ID is tested on ImageNet, and OOD is averaged over $5$ ImageNet variations. Experiments with $[1,2,4]$-shots are presented. Each accuracy is averaged over $3$ runs. We can see that our proposed method overwhelms WISE-FT in all cases.}
        \label{fig:id_ood_curve_avg_ft}
\end{figure}


%Its non-smoothness makes it notoriously hard for auto-differentiation. To circumvent the smoothness issue, we apply the GPU implementation \citep{wong2021leveraging} of a variance-reduction proximal gradient method SAGA \citep{defazio2014saga}. As a side node, $\ell_1$ encourages $\mW\_{avd}$ to have a small number of non-zero entries, which implies that for any fixed class, we only use a small number of semantic features. One could also use $\ell_{2,1}$ norm for robust feature selection \citep{nie2010efficient}. The subtle difference is that $\ell_{2,1}$ norm will encourage the classification of different class to share the \textsl{same} group of features. 


%\begin{table*}[h!]
%\centering
% \begin{tabular}{l|cccccc} 
% \midrule
%\quad Shots & IN & IN-R & IN-A & IN-V2 & IN-Sketch & ObjectNet\\
%\midrule
%$k=1$, LP & 76.97 & 89.11 & 77.78 & 71.25 & 60.89 & 68.82 \\
%$k=1$, AVD & 77.57 & 89.39 & 78.30 & 72.02 & 61.36 & 69.22 \\
% \midrule
%$k=2$, LP & 78.55 & 89.37 & 78.09 & 72.18 & 61.30 & 69.11 \\
%$k=2$, AVD & 79.12 & 89.51 & 78.44 & 72.82 & 61.80 & 69.33 \\
% \midrule
%$k=4$, LP & 79.67 & 89.41 & 78.33 & 72.90 & 61.49 & 69.11 \\
%$k=4$, AVD & 79.99 & 89.64 & 78.57 & 73.47 & 61.98 & 69.36 \\
% \midrule
%$k=8$, LP & 80.82 & 89.51 & 78.59 & 73.69 & 61.76 & 69.44 \\
%$k=8$, AVD & 81.00 & 89.63 & 78.62 & 74.20 & 62.16 & 69.58 \\
% \midrule
%$k=16$, LP & 81.86 & 89.56 & 78.56 & 74.19 & 61.88 & 69.38 \\
%$k=16$, AVD & 81.75 & 89.63 & 78.79 & 74.66 & 62.30 & 69.51 \\
%\midrule
%$k=32$, LP & 81.86 & 89.56 & 78.56 & 74.19 & 61.88 & 69.38 \\
%$k=32$, AVD & 81.75 & 89.63 & 78.79 & 74.66 & 62.30 & 69.51 \\
% \bottomrule
% \end{tabular}
% \caption{Accuracies on ImageNet and its variation. We compare linear probing with image features vs sparse logistic regression with AVDs.}
% \label{table:fs_comparison}
%\end{table*}

\begin{table*}[h!]
\centering
 \caption{Accuracies on ImageNet and its variation. We compare LP vs SLR-AVD.}

\resizebox{\columnwidth}{!}{
 \begin{tabular}{c|cc|cc|cc|cc|cc|cc} 
 \midrule
 Shots & \multicolumn{2}{c|}{$k=1$}  &  \multicolumn{2}{c|}{$k=2$} & \multicolumn{2}{c|}{$k=4$}&  \multicolumn{2}{c|}{$k=8$} &  \multicolumn{2}{c|}{$k=16$} &  \multicolumn{2}{c}{$k=32$} \\
 \midrule
 Methods & LP & AVD & LP & AVD  & LP & AVD &  LP & AVD &  LP & AVD &  LP & AVD \\
 \midrule
IN & 31.51 & \bf 40.56 & 44.06 & \bf 54.16 & 54.66 & \bf 63.19 & 62.33 & \bf 68.23 & 67.55 & \bf 71.40 & 71.15 & \bf 73.67 \\
IN-R & 35.23 & \bf 48.88 & 46.30 & \bf 61.23 & 54.50 & \bf 67.64 & 59.25 & \bf 70.58 & 62.16 & \bf 72.54 & 64.32 & \bf 74.53 \\
IN-A & 22.52 & \bf 29.81 & 27.26 & \bf 36.96 & 32.34 & \bf 42.09 & 34.88 & \bf 44.41 & 36.68 & \bf 45.15 & 39.19 & \bf 47.89 \\
IN-V2 & 26.91 & \bf 35.12 & 37.13 & \bf 47.07 & 45.92 & \bf 55.02 & 52.50 & \bf 59.15 & 57.62 & \bf 62.52 & 61.23 & \bf 64.75 \\
IN-Sketch & 16.80 & \bf 22.87 & 21.96 & \bf 31.03 & 28.77 & \bf 37.43 & 33.29 & \bf 40.73 & 35.62 & \bf 42.94 & 38.64 & \bf 45.39 \\
ObjectNet & 19.38 & \bf 25.43 & 24.98 & \bf 34.11 & 32.44 & \bf 40.39 & 36.02 & \bf 42.80 & 41.50 & \bf 45.82 & 43.67 & \bf 49.17 \\
\midrule
Average $\uparrow$ & \multicolumn{2}{c|}{8.39} & \multicolumn{2}{c|}{10.48} & \multicolumn{2}{c|}{9.52} & \multicolumn{2}{c|}{7.94} & \multicolumn{2}{c|}{6.54} & \multicolumn{2}{c|}{6.20} \\
 \bottomrule
 \end{tabular}
 }
 \label{table:fs_comparison}
\end{table*}



For simplicity, we will use the following acronyms for different methods and datasets. We defer the hyperparameter discussions to the appendix.

\noindent\textbf{ZS:} Zero-shot classification using text embeddings of hand-crafted prompts ensembles. 
\noindent\textbf{ZS-VD, ZS-AVD:} Zero-shot classification using visual descriptor and augmented visual descriptors, respectively.
\noindent\textbf{LP:} Linear probing using image embeddings.
\noindent\textbf{SLR-AVD:} Sparse logistic regression using AVDs. 
\noindent\textbf{FT:} Finetuning the image encoder and classification head.
\noindent\textbf{SLR-FT-AVD:} Sparse logistic regression with AVD, and then finetune the linear head plus the image encoder with frozen sparsity patterns.
\noindent\textbf{WISE-FT:} Weight ensemble using ZS and FT.
\noindent\textbf{WISE-SLR:} Weight ensemble using SLR-FT-AVD and ZS-AVD. 
\noindent\textbf{IN:} ImageNet.
\noindent\textbf{IN-R:} ImageNet-R.
\noindent\textbf{IN-A:} ImageNet-A.
\noindent\textbf{IN-V2:} ImageNetV2.
\noindent\textbf{IN-Sketch:} ImageNet-Sketch.
%
%\paragraph{Hyperparameter} For ImageNet and its variations, we fix a set of 6804 augmented visual descriptors. The hyperparameters are swept over disjoint training and validation sets of size $20$ per class for LP and SLR-AVD. For $\ell_1$ regularization, its non-smoothness makes it notoriously hard for auto-differentiation. To circumvent the smoothness issue, we apply the GPU implementation \citep{wong2021leveraging} of a variance-reduction proximal gradient method SAGA \citep{defazio2014saga}.
%We adopt the \textit{regularization path} approach, in which the solver optimizes over $100$ regularization strengths $\lambda_1>\lambda_2\cdots >\lambda_{100}$. Here we set $\lambda_1$ to be the strength that returns a model that uses none of the features, and $\lambda_{100}=0.1\times\lambda_1$. For LP, we always use $\ell_2$ regularization, we use L-BFGS implemented by scikit-learn, and search for the regularization strength over $100$ grids between $0.5$ and $6$. All the $\lambda$s are evenly spread in the log-space\footnote{In python numpy.logspace(math.log10($\lambda_1$), math.log10($\lambda_{100}$), 100)}. For FT and SLR-FT-AVD, we select hyperparameters using a training and validation set of size $4$ per class. The batch size is fixed to be $512$ and the number of epochs is fixed to be $10$. We always optimize with AdamW, and choose a cosine rate scheduler with warm-ups. We randomly select learning rate in $[1e-8, 3e-5]$, weight decay in $[0.1, 0.12]$, and warm up steps in $\{0, 50, 500\}$, for $20$ trials. The chosen parameters are then fixed throughout all experiments. 



\subsection{Zero-shot with AVDs}
As mentioned in \cref{subsec:genvd}, we can easily establish zero-shot matrices with AVDs. We set $\mW\_{vd}$ to be the aforementioned block diagonal form, $\mW\_{cp}$ to be an identity matrix. We merge them into $\mW\_{avd}=[\mW\_{vd}, \gamma\mW\_{cp}]$.
 Their performances are compared in \cref{table:zs_comparison}. ZS-AVD outperforms every zero-shot baseline on all ImageNet variations. We find that simply using VD usually underperforms ZS, indicating that the class names are probably one of the strongest prompts. This observation is intuitive as during contrastive training, the class name itself is likely to show up in the caption the most often, compared to other visual descriptors. 
 One can certainly try to improve ZS-VD results by more carefully prompting GPT-3, or gathering descriptors from different data sources/search engines. \citet{pratt2022does,yang2022language,menon2022visual} have studied the quality of descriptors across different datasets and hyperparameters (e.g. temperature for sampling, etc) settings. Here we did not further pursue that path. Instead, we realize that simply using the merged prompts $\mW\_{avd}$ already surpasses the best zero-shot classifier. Notice here we have a parameter $\gamma$ that decides how important we weigh the zero-shot model. Empirically we find that setting $\gamma=5$ is sufficient for all datasets.
 \anna{Here, we do not further pursue this direction. Instead, we utilize our observation that simply using the merged prompts $\mW\_{avd}$ already surpasses the best zero-shot classifier. Our only (?) parameter is $\gamma$ which determines how much to weight the zero-shot model. Empirically we find that setting $\gamma=5$ is sufficient for all datasets.}


\subsection{Comparison to linear probing}

We compare SLR-AVD to LP with shot $[1,2,4,8,16,32]$ per class. \anna{$\{1,2,4,8,16,32]\}$ shots per class} Each experiment is conducted 3 times with independent random seeds. We report the averaged test accuracy on ImageNet and its distribution shift variations, see \cref{fig:fs_comparison} for details. Our proposed method outperforms linear probing on all tasks. Detailed accuracies are presented in \cref{table:fs_comparison}. In a nutshell, our method outperforms linear probing by $8.39\%$, $10.48\%$, $9.52\%$, $7.94\%$, $6.54\%$, $6.20\%$ on $k=1,2,4,8,16,32$ respectively.

%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/fs_img_vs_text_avg.pdf}
%     \end{subfigure}
%
%        \caption{Few-shot experiments compare learning with augmented visual descriptors (AVD) vs linear probing. In each subfigure, the y-axis represents the number of shots per class. Here we consider shot in $[1,2,4,8,16,32]$ per class. The accuracies are averaged over all six ImageNet and its variation datasets, and over 3 runs. Learning with AVD is significantly more sample efficient in both in-distribution and out-of-distribution tasks.}
%        \label{fig:fs_comparison}
%\end{figure}




Although learning with visual descriptors significantly outperforms linear probing in the few-shot setting, we should remark that ImageNet and its variations are usually considered ``in-distribution'' to the CLIP training data. In this case, the zero-shot model itself is usually a very strong baseline, and they typically outperform these few-shot models, as one can compare \cref{table:zs_comparison} and \cref{table:fs_comparison}. \anna{In this case, the zero-shot model itself is usually a very strong baseline, and typically outperforms few-shot models, as can be observed by comparing the results in tables \cref{table:fs_comparison} and \cref{table:zs_comparison}.} WISE-FT serves as a strong method to improve both in-distribution and out-of-distribution accuracies. \anna{I might clarify here that this can be used for any of the settings, i.e. SLR-AVD, LP, VD, etc. before you get into it so people aren't confused by a "learned" subscript vs a "VD" subscript etc} In particular, we can train a linear head $\mW\_{learned}$, and interpolate with the zero-shot weight  $\mW\_{zs}$ by taking a convex combination $\alpha\mW\_{zs}+(1-\alpha)\mW\_{learned}$, for $\alpha=\{\alpha_1,\ldots, \alpha_n\}$. We are free to vary $\alpha$. Then for each $\alpha_i$, we can plot that weight ensemble's in-distribution and out-of-distribution test accuracy.  This procedure thus creates an ID-OOD frontier and along the curve, some ensemble excels at both ID and OOD distribution. We further show that with WISE-FT, our method still dominates the WISE-FT with image features. \anna{Is this like a WISE-FT of SLR-AVD vs a WISE-FT of VD? Consistent terminology here might help.} See the ID-OOD curves in \cref{fig:id_ood_curve_avg}. We show the plot of $k=4,8,16$. SLR-AVD's ID-OOD curve overwhelms that of LP, indicating that SLR-AVD is better at both ID and OOD tasks. 

\subsection{Comparison to finetuning}
\anna{What does this sentence mean? Specifically the "WISE-FT the whole image encoder" Also WISE-SLR isn't defined} We compare WISE-FT the whole image encoder to WISE-SLR. The ID-OOD frontier is presented in \cref{fig:id_ood_curve_avg_ft} and the accuracies are reported in \cref{table:optimal_alpha_ft}.  

On in-distribution task, WISE-SLR outperforms vanilla WISE-FT by $1.43\%$, $1.62\%$, and $1.61\%$ respectively with $k=1,2,4$ shot training data. Averaging over $5$ distribution shift datasets, with optimal $\alpha$, WISE-SLR outperforms vanilla WISE-FT by $0.88\%$, $0.73\%$, and $0.64\%$ respectively with $k=1,2,4$. The optimal $\alpha$ is picked independently for each method on each dataset. 



\subsection{Comparison to CoOp}
We compare linear probing with AVD to CoOp \citep{zhou2022learning} as well. CoOp learns the prefix of ``\texttt{[prefix] classname}'' \anna{should we say something like ``\texttt{\{classname\}}'' instead if it uses the actual classname?} in the continuous token embedding space. The benefit of CoOp is that it operates in a continuous space, hence one can optimize using standard backpropagation, and it is quite sample efficient. On the other hand, due to the requirement of backprop, CoOp stores a large computation graph, hence memory-efficiency is a big advantage of SLR-AVD over CoOp.

When implementing CoOp, we choose a prefix of length $16$ and do not use a suffix. The prefix is fixed for all classes. We train with Adam for 20 epochs, setting the batch size to 512. This gives us comparable results to those of the original paper. 

Since CoOp injects ``\texttt{classname}'' to the prompt during inference directly, this enforces a very strong prior. For a fair comparison, we also inject a strong prior by interpolating our learned linear head $\alpha \mW\_{avd} + (1-\alpha) \mW\_{zs}$ with the zero-shot linear classifier. We use $\alpha=0.05k$ where $k$ is the number of shots. Resnet-50 vision backbone is used for both methods. See the result in \cref{table:avd_vs_coop}. SLR-AVD exceeds CoOp by $1.73$, $1.49$, $1.55$, $1.53$, $1.95$ on $k=1,2,4,8,16$, respectively. 

 \begin{table}
\begin{minipage}[t]{0.4\textwidth}\vspace{0pt}\centering
 \caption{Accuracies of zero-shot, visual descriptors, and augmented visual descriptors on ImageNet and its variation. ZS-AVD outperforms all baselines across different datasets.}
\resizebox{\columnwidth}{!}{
 \begin{tabular}{c|ccc} 
 \toprule
 & ZS & ZS-VD & ZS-AVD \\
 \midrule
 IN & 68.78 & 65.89 & \bf 69.52\\ 
 IN-V2 & 62.23 & 59.19 & \bf 62.97\\ 
 IN-R & 77.72 & 72.75 & \bf 77.85\\ 
 IN-A & 50.64 & 46.11 &\bf  50.87\\ 
 IN-Sketch & 48.38 & 44.84 & \bf 48.91\\ 
 ObjectNet & 54.31 & 49.60 &\bf  54.58\\ 
 \bottomrule
 \end{tabular}
 }
 \label{table:zs_comparison}
\end{minipage}
  \hfill
  \begin{minipage}[t]{0.55\textwidth} \label{table:avd_vs_coop}
    \centering
      \caption{Accuracies of CoOp and SLR-AVD on ImageNet. For SLR-AVD, we interpolate the learned weights with zero-shot weights by $\alpha \mW\_{avd} + (1-\alpha) \mW\_{zs}$, where $\alpha=0.05k$ and $k$ is the number of shot per class.}
      \resizebox{\columnwidth}{!}{
		 \begin{tabular}{c|ccccc} 
		 \toprule
		 Shots & 1 & 2 & 4 & 8 & 16\\
		\midrule
		CoOp & 59.54 & 60.23 & 60.97 & 62.20 & 63.02 \\
		AVD & 61.27 & 61.72 & 62.52 & 63.73 & 64.97  \\
		$\Delta$ & +1.73 & +1.49 & +1.55 & +1.53 & +1.95\\
		
		 \bottomrule
		 \end{tabular}
	}
    \end{minipage}
  \end{table}

%\begin{table}[h]
%\centering
% \caption{Accuracies of CoOp and SLR-AVD on ImageNet. For SLR-AVD, we interpolate the learned weights with zero-shot weights by $\alpha \mW\_{avd} + (1-\alpha) \mW\_{zs}$, where $\alpha=0.05k$ and $k$ is the number of shot per class.}
% \begin{tabular}{c|ccccc} 
% \midrule
% Shots & 1 & 2 & 4 & 8 & 16\\
%\midrule
%CoOp & 59.54 & 60.23 & 60.97 & 62.20 & 63.02 \\
%AVD & 61.27 & 61.72 & 62.52 & 63.73 & 64.97  \\
%$\Delta$ & +1.73 & +1.49 & +1.55 & +1.53 & +1.95\\
%
% \bottomrule
% \end{tabular}
%
% \label{table:avd_vs_coop}
%\end{table}






